Data-Driven Identification of Attack-free Sensors in Networked Control Systems

This paper proposes a data-driven framework to identify the attack-free sensors in a networked control system when some of the sensors are corrupted by an adversary. An operator with access to offline input-output attack-free trajectories of the plant is considered. Then, a data-driven algorithm is proposed to identify the attack-free sensors when the plant is controlled online. We also provide necessary conditions, based on the properties of the plant, under which the algorithm is feasible. An extension of the algorithm is presented to identify the sensors completely online against certain classes of attacks. The efficacy of our algorithm is depicted through numerical examples.

==> Archive/App-27Nov2023.tex <==
\subsection{Proof of Lemma \ref{lem:data_OL}}\label{app3}
To help us prove Lemma \ref{lem:data_OL}, we next provide two intermediate results.
\begin{lemma}\label{lem:SS_ARX}
Consider a controllable and observable DT LTI SS model defined by the tuple $\Sigma \triangleq (A,B,C,0)$. Let $y[k] \in \mathbb{R}^m, u[k] \in \mathbb{R}^m, x[k] \in \mathbb{R}^n$ represent the output signal, input signal, and state signal. Then there exists an equivalent ARX model denoted by 
    \begin{equation}\label{ARX}
    y[k]+\Upsilon_{n}z[k-1]+\dots+\Upsilon_{1}z[k-n]=\Pi_{n}u[k-1]+\dots + \Pi_{1}u[k-n]. \qquad \square
\end{equation}
\end{lemma}
The proof of Lemma \ref{lem:SS_ARX} is well established (see \citet[Chapter 4]{antsaklis1997linear}, and \citet[Section II.B]{wu2022equivalence}) and thus is omitted. We next recall a result from \citet[Theorem 1]{de2019formulas}.
\begin{lemma}\label{lem:data_de_persis}
Consider a controllable and observable DT LTI SS model defined by the tuple $\Sigma \triangleq (A,B,C,0)$. Let $y[k] \in \mathbb{R}^m, u[k] \in \mathbb{R}^m, x[k] \in \mathbb{R}^n$ represent the output signal, input signal, and state signal. Then, if $\text{rank}\begin{bmatrix}
    U_{0,1,T}\\X_{1,T}
\end{bmatrix}=n+m$, then the state space model has an equivalent representation 
\begin{equation}
    x[k+1] = X_{1,T}\begin{bmatrix}
    U_{0,1,T}\\
        X_{0,T}
    \end{bmatrix}\ssymbol{2} \begin{bmatrix}
    u[k]\\
        x[k]
    \end{bmatrix}. \quad \square
\end{equation}
\end{lemma}
Using the above two results, we now begin to prove Lemma \ref{lem:data_OL}.
% Consider the SS representation in \eqref{eq:SS_con_form}. Then, from \cite[Chapter 3]{antsaklis1997linear}, we can derive an equivalent SS representation of \eqref{eq:SS_con_form} in controller form. Let the system matrices in controller form be represented by the tuple $(A_{c,j},B_{c,j},C_{c,j},D_{c,j})$. Let $\mu_i,i\in \{1,\dots,m\}$ be the controllability indices of the system  (see \cite[Section 3.4.D]{antsaklis1997linear} for the definition of controller form, and \cite[Definition 4.1]{antsaklis1997linear} for the definition of controllability indices). Then, Lemma \ref{lem:SS_PMS} follows from \cite[(3.26)]{antsaklis1997linear}.
% \begin{lemma}\label{lem:SS_PMS}
%     Let $q$ represent the DT shift operator. Let the matrix $S(q)$ be defined as follows
%     \begin{equation}
%         S(q) = \textbf{blockdiag}[(1,q,\dots,q^{\mu_i})], i\in \{1,\dots,m\}.
%     \end{equation}
%     Let $N_j(q)$ and $D_j(q)$ be polynomial matrices which satisfy the following equality
%     \begin{equation}\label{eq:PMD_SS}
%         \begin{bmatrix}
%             B_{c,j} & 0\\D_{c,j} & I_g
%         \end{bmatrix}\begin{bmatrix}
%             D_j(q) & I_m\\
%             -N_j(q) & 0
%         \end{bmatrix}=\begin{bmatrix}
%             qI_n-A_{c,j} & B_{c,j} \\-C_{c,j} & D_{c,j}
%         \end{bmatrix}\begin{bmatrix}
%             S(q) & 0\\0 & I_m
%         \end{bmatrix}
%     \end{equation}
%     with the additional constraints that $(B_{c,j},qI-A_{c,j})$ are left co-prime and $(D_j(q),S_j(q))$ are right co-prime. Then the SS representation \eqref{eq:SS_con_form}
%     and the PMD representation $z_j[k]=N_j(q)D_j(q)^{-1}u[k]$ are equivalent. $\hfill \square$
% \end{lemma}
% The above lemma states that, any controllable SS model can be converted into an equivalent PMD model. Since the PMD model is expressed using the shift operator form, it can be converted to an equivalent ARX form. Thus, using the result of Lemma \ref{lem:SS_PMS}, we write the ARX form of the SS plant in \eqref{eq:SS_con_form} as
% \begin{equation}\label{ARX}
%     z_j[k]+\Upsilon_{j,n}z_j[k-1]+\dots+\Upsilon_{j,1}z_j[k-n]=\Pi_{{j,n}}u[k-1]+\dots + \Pi_{j,1}u[k-n]
% \end{equation}
% where $j \in \{1,\dots,{N \choose Q}\}$. $\hfill \square$

\textit{Proof of Lemma \ref{lem:data_OL}:} Consider the SS model in \eqref{eq:SS_con_form}. Using the results of Lemma \ref{lem:SS_ARX}, we know that for the SS model \eqref{eq:SS_con_form}, there exists an equivalent ARX model as follows
 \begin{equation}\label{ARX}
    z_j[k]+\Upsilon_{j,n}z_j[k-1]+\dots+\Upsilon_{j,1}z_j[k-n]=\Pi_{{j,n}}u[k-1]+\dots + \Pi_{j,1}u[k-n],\; \forall j \in \Omega
\end{equation}
Using the definition of states $\mathcal{X}_j$ in \eqref{data_matrices0}, we formulate an equivalent state space formulation as
\begin{equation}\label{eq:CL}
\mathcal{X}_j[k+1]=\bar{A}_j\mathcal{X}_j[k] +\bar{B}u[k],
\end{equation}
where $\setlength{\dashlinegap}{0.8pt}\left[\begin{array}{c:c}
  \bar{A}_j   & \bar{B}
\end{array}\right] \triangleq $
\begin{equation}\label{eq:A_B}
\setlength{\dashlinegap}{0.8pt}
\left[\begin{array}{cccccccccc:c}
0 & I & 0 & \dots & 0 & 0 & 0 & 0 & \dots & 0 & 0\\
0 & 0 & I & \dots & 0 & 0 & 0 & 0 & \dots & 0 & 0\\
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots  & \vdots\\
0 & 0 & 0 & \dots & I & 0 & 0 & 0 & \dots & 0 & 0\\
-\Upsilon_{j,n}& -\Upsilon_{j,n-1} & -\Upsilon_{j,n-2} & \dots & -\Upsilon_{j,1} & \Pi_{j,n} & \Pi_{j,n-1} & \Pi_{j,n-2} & \dots & \Pi_{j,1}  & 0\\
\hdashline
0 & 0 & 0 & \dots & 0 & 0 & I  & 0 & \dots & 0 & 0\\
0 & 0 & 0 & \dots & 0 & 0 & 0  & I & \dots & 0 & 0\\
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots\\
0 & 0 & 0 & \dots & 0 & 0 & 0  & 0 & \dots & I & 0\\
0 & 0 & 0 & \dots & 0 & 0 & 0  & 0 & \dots & 0 & I
\end{array}\right]
\end{equation}
Note here that, the input-output data that was collected in $\mathcal{I}_T$ obeys the dynamics in \eqref{eq:CL}. In other words, we have now constructed a state space representation with access to input and state data. Then the proof follows from Lemma \ref{lem:data_de_persis} $\hfill \blacksquare$
% \subsection{Numerical example depicting the relation between SS, PMD and ARX model}\label{Sec:app1}
% Consider the matrices 
%     \begin{equation}
%         A_c=\begin{bmatrix}
%         0 & 1 & 0\\
%         0 & 0 & 1\\
%         2 & 1 & -2
%     \end{bmatrix},\;
%     B_c= \begin{bmatrix}
%         0 \\ 0 \\ 1
%     \end{bmatrix},\;
%     C_c= \begin{bmatrix}
%         0 \\ 1 \\ 0
%     \end{bmatrix}^T
%     \end{equation}
%  which are in the controller form. The corresponding PMD matrices obtained from \eqref{eq:PMD_SS} are $N(q)=q$ and $D(q)=q^3+2q^2-q-2$. Then 
%  \begin{align}
%      &z[k]=\frac{q}{q^3+2q^2-q-2}u[k]\\
%      &z[k+3]+2z[k+2]-z[k+1]-z[k]=u[k+1]\\
%      &z[k]=2z[k-1]+z[k-2]+z[k-3]+u[k-2]
%  \end{align}
%  where the last equation is in the ARX form similar to \eqref{ARX}.$\hfill \square$
\subsection{Proof of Lemma \ref{lem:rank_obsv}}\label{app2}
For any given $j \in \left\{1,2,\dots,{N \choose Q}\right\}$, it holds from \eqref{data_matrices0} that 
\begin{equation}\label{e1}
    \underbrace{\begin{bmatrix}
        U_{n,T}\\
        \hline
        \hat{X}_{j,n,T}
    \end{bmatrix}}_{M_0}=\begin{bmatrix}
        U_{n,T}\\
        \hline 
        Z_{j,0,n,T}\\
        U_{0,n,T}
    \end{bmatrix}, \quad 
    \text{where}\quad 
    Z_{j,0,n,T} = \underbrace{\begin{bmatrix}
         \mathcal{O}_{j,n} & \mathcal{T}_{j,n}
    \end{bmatrix}}_{M_1} \underbrace{\begin{bmatrix}
        X_{0,T}\\
        U_{0,n,T}
    \end{bmatrix}}_{M_2}
\end{equation}
where the matrix $X_{0,T}$ is defined similar to \citet[(4)]{de2019formulas}, and $
\left[\begin{array}{c|c}
\mathcal{O}_{j,n} & \mathcal{T}_{j,n}
\end{array}\right]=$
\begin{equation}\label{e0}
\left[\begin{array}{c|cccc}
        C_{\bar{\mathcal{J}}_{Q,j}} & 0 & 0 & \dots & 0\\
        C_{\bar{\mathcal{J}}_{Q,j}}A & C_{\bar{\mathcal{J}}_{Q,j}}B & 0& \dots & 0\\
        C_{\bar{\mathcal{J}}_{Q,j}}A^2 & C_{\bar{\mathcal{J}}_{Q,j}}AB & C_{\bar{\mathcal{J}}_{Q,j}}B& \dots & 0\\
        \vdots & \vdots & \vdots & \ddots & \vdots\\
        C_{\bar{\mathcal{J}}_{Q,j}}A^{n-1} & C_{\bar{\mathcal{J}}_{Q,j}}A^{n-2}B & C_{\bar{\mathcal{J}}_{Q,j}}A^{n-3}B & \dots & 0
\end{array}\right]
\end{equation}
The matrix $M_0$ is of dimension $M_0 \in \mathbb{R}^{s \times T}$ where $s \triangleq m(n+1)+Qn$. We aim to show that condition \eqref{eq:PE}, or equivalently the condition 
\begin{equation}\label{rank}
\text{rank}(M_0)=s,
\end{equation}
does not hold when the tuple $(A,C_{\bar{\mathcal{J}}_{Q,j}})$ is not observable. From the theorem statement, since we know that $T > m(n+1)+Qn$, we observe that $M_0$ is a fat matrix (more columns than rows). Thus, the condition \eqref{rank} holds only if $M_0$ has full row rank $s$. From \eqref{e1}, one of the necessary conditions for \eqref{rank} to hold is
\begin{equation}\label{e3}
    \text{rank}(Z_{j,0,n,T})= nQ. 
\end{equation}
Using \eqref{e1}, \eqref{e3} is rewritten as 
\begin{equation}\label{f1}
 \text{rank}(Z_{j,0,n,T})= \min \{\text{rank}(M_1),  \text{rank}(M_2)\} =nQ
\end{equation}
From \citet[Lemma 1]{de2019formulas} we know that for any controllable system where the input is persistently exciting of order $(m+Q)n+1$, it holds that $\text{rank}(M_2) = n(m+1)$, i.e., $M_2$ is of full rank. Then \eqref{f1} can be re-writtten as
\begin{equation}\label{e5}
\min \{\text{rank}(M_1),n(m+1)\} = nQ
\end{equation}
where $M_1 \in \mathbb{R}^{Qn \times n(m+1)}$. We next show that condition \eqref{e5} (which is a necessary condition for \eqref{e3} to hold) cannot hold when the tuple $(A,C_{\bar{\mathcal{J}}_{Q,j}})$ is not observable. 

First, consider the case that $Q > m+1$. Then $rank (M_0) \neq nQ$ since the rank cannot be larger than the smallest dimension of the matrix. Second, consider the case that $Q = m+1$. Then $rank (M_0) = nQ$, only if the matrix $M_0$ has full rank. However, we observe that there is a zero column in $M_0$ which reduces the rank. 

Finally, we consider the case that $Q< m+1$. Then, 
% since $M_1 \in \mathbb{R}^{Qn \times n(m+1)}$, 
if the tuple $(A,C_{\bar{\mathcal{J}}_{Q,j}})$ is not observable, $\text{row\;rank}(\mathcal{O}_{j,n}) \leq n-1$. Let this be observation O1. Consider the matrix $\mathcal{T}_{j,n} \in \mathbb{R}^{nQ \times nm}$. Since one of the rows of $\mathcal{T}_{j,n}$ is zero, the maximum row rank that the matrix $\mathcal{T}_{j,n}$ can attain is $nQ-Q$. Let this be observation O2. Combining O1 and O2, the maximum row rank of $M_0$ is the sum of the row ranks of $\mathcal{O}_{j,n}$ and $\mathcal{T}_{j,n}$. That is, $\max \text{rank}(M_0) \leq n-1+nQ-Q$. Plugging this inequalities in the L.H.S of \eqref{e5}, we get
\begin{equation}\label{e6}
    \text{rank}(Z_{j,0,n,T}) = \min\{nQ+n-Q-1, n(m+1)\},
\end{equation}
From the Lemma statement, $n < Q+1 \implies n-Q-1 <0$, then 
\begin{equation}\label{e7}
 nQ < n-1+nQ-Q.    
\end{equation}
Substituting \eqref{e7} into \eqref{e6}, we get $\text{rank}(Z_{j,0,n,T}) < nQ$
which concludes the proof. $\hfill \blacksquare$
\subsection{Proof of Proposition \ref{prop1}}\label{app5}
Let us consider the data-based representation of the plant in \eqref{data:OL}. Algorithm \ref{alg1} states that, for any given input, if the received output data of the plant and the output of the data-based representation are the same, then the sensor is attack-free. The proof follows by observing that, under sensor attacks, there is a direct feed-through term from the attack input to the measurement output. That is, the relationship between the attacked input and the measurement output can be written as
\begin{align}
    x[k+1]&=Ax[k]+Bu[k]\\
    z_j[k]&=C_{\bar{\mathcal{J}}_{Q,j}}x[k] + \omega_j[k], j \in \{1,\dots,{N \choose Q}\}
\end{align}
where $\omega_j[k]$ is the stacked projection of the attack vector. Then, the sensor output $z_j[k]$ \textit{must} be different from the predicted output (using the model-based representation) if and only if there is a non-zero attack on the sensors. This concludes the proof. $\hfill \blacksquare$
\subsection{Proof of Lemma \ref{lem:replay}}\label{App6}
Consider the plant under replay attacks \eqref{replay}. Now, let us consider the rank condition 
\begin{equation}\label{t1}
    \text{rank}\begin{bmatrix}
        \underline{U}_{k+n,T_1},\\ \underline{\hat{X}}_{j,k+n,T_1},
    \end{bmatrix}=m(n+1)+Qn,
\end{equation}
As shown in the proof of Lemma \ref{lem:rank_obsv}, a necessary condition  for \eqref{t1} to hold is
\begin{equation}\label{t2}
    \text{rank}(\underline{Z}_{j,0,n,T})= nQ, 
\end{equation}
when $k=0$.The matrix $\underline{Z}_{j,0,n,T}$ is a fat matrix and satisfies \eqref{t2} only if it has full row rank. To inspect the row rank, let us rewrite $\underline{Z}_{j,0,n,T}$ as 
\begin{equation}
\begin{bmatrix}
        z_j[0]\vert_{1} & z_j[1]\vert_1 & \dots & z_j[T-1]\vert_{1}\\
        z_j[1]\vert_{1} & z_j[2]\vert_{1} & \dots & z_j[T]\vert_{1}\\   
        \vdots & \vdots & \ddots & \vdots\\
        z_j[n-1]\vert_{1} & z_j[n]\vert_{1} & \dots & z_j[n-1+T]\vert_{1}
    \end{bmatrix}
\end{equation}
where $\vert_{1}$ denotes that under replay attack, at least one of the rows of $z_j[\cdot]$ is a constant $c_j$. Then at least $n$ rows of the matrix are constants which makes the matric row rank deficient. This concludes the proof. $\hfill \blacksquare$

==> Archive/Identification-05Nov23-Sri.tex <==
We first derive a data-driven representation of the plant \eqref{P} offline, which gives us a data-driven open loop model that explains the input and output trajectories of length $T$, $\mathcal{I}_{T}$. 

\subsection{Learning the data-driven open-loop (offline) model}
Due to Assumption \ref{assum:M-attacks}, we know that at most $M$ sensors can be compromised, but we do not know which sensors have been compromised. Hence, our approach is to learn the open-loop models of the plant with every subset of $N-M$ sensors. In other words, we will learn to total of $(N-M)$-combination data-driven open-loop models from the data $\mathcal{I}_{T}$. To this end, let the plant \eqref{P} with output $z_j[k]$ for $j \in \left\{1,\dots,{N \choose N-M}\right\}$, be described as follows
\begin{equation}\label{eq:SS_con_form}
x[k+1]=Ax[k]+Bu[k], \quad z_j[k]=C_{{\mathcal{J}}_{j}}x[k], \; k\in\mathbb{Z},
\end{equation}
where ${\mathcal{J}}_{j}\subset \{1,\dots,N\}$ with cardinality $N-M$ and $C_{{\mathcal{J}}_{j}}$ is a matrix obtained by stacking all the matrices $C_i$ for $i\in {\mathcal{J}}_{j}$. Note that \eqref{P} and \eqref{eq:SS_con_form} are equivalent since their input and output trajectories match. Necessarily, we assume the following 
\begin{assumption}[$N-M$-sensor observability]\label{assum:q_sen_obsv}
For every subset $\mathcal{J}\subset \{1\dots,N\}$ with cardinality $N-M$, the tuple $(A,C_{\mathcal{J}})$ is observable where $C_{\mathcal{J}}$ is a matrix obtained by stacking the matrices $C_i,i\in \mathcal{J}$. $\hfill \triangleleft$
\end{assumption}
We say that the plant \eqref{P} is $(N-M)$-sensor observable when Assumption \ref{assum:q_sen_obsv} holds. Therefore, every $j\in\left\{1,\dots,{N \choose N-M}\right\}$ model described by \eqref{eq:SS_con_form} is observable. To construct a data-based representation of the plant \eqref{eq:SS_con_form} (or equivalently \eqref{P}) using $\mathcal{I}_{T}$, define 
\begin{equation}\label{data_matrices0}
\hat{X}_{j,n,T} \triangleq  \begin{bmatrix}
        Z_{j,0,n,T}\\
        \hline 
        U_{0,n,T}\\
    \end{bmatrix},\; \mathcal{X}_{j}[k]^T \triangleq
\setlength{\dashlinegap}{0.5pt}
\begin{bmatrix}[ccc:ccc] z_{j}^T[k-n]&...&z_j^T[k-1]& u^T[k-n]&...& u^T[k-1]\end{bmatrix}.
\end{equation}
Then the operator constructs the following matrices from the data. 
\begin{align}
    U_{n,T}&=\begin{bmatrix}
        u[n] & u[n+1]& \dots & u[n+T-1]
    \end{bmatrix} \label{data_matrices}\\
    \hat{X}_{j,n,T}&=\begin{bmatrix}
        \mathcal{X}_{j}[n] & \mathcal{X}_{j}[n+1]& \dots & \mathcal{X}_{j}[n+T-1]
    \end{bmatrix} \label{data_matrices1}\\
    \hat{X}_{j,n+1,T}&=\begin{bmatrix}
        \mathcal{X}_{j}[n+1] & \mathcal{X}_{j}[n+2]& \dots & \mathcal{X}_{j}[n+T]
    \end{bmatrix} \label{data_matrices2}
\end{align}
Note that the state $\mathcal{X}_j$ in contains the history of past inputs and past outputs of length $n$. Thus there is an offset of length $n$ whilst constructing the data matrices \eqref{data_matrices}. Now the following result is obtained using \citet[Theorem 1, Lemma 2]{de2019formulas}.
\begin{lemma}\label{lem:data_OL}
For any given $j \in \left\{1,\dots,{N \choose N-M}\right\}$, let
\begin{equation}\label{eq:PE}
    \text{rank}\begin{bmatrix}
        U_{n,T}\\\hat{X}_{j,n,T}
    \end{bmatrix}=m(n+1)+(N-M)n,
\end{equation}
with $T\geq (m+1)\tilde{n}$ where $\tilde{n}\triangleq (m+N-M)n+1$. Then \eqref{eq:SS_con_form} has the equivalent data-driven representation in \eqref{data:OL}, where $\ssymbol{2}$ denotes the right inverse.
\begin{equation}\label{data:OL}
\mathcal{X}_j[k+1]=\Lambda_j\begin{bmatrix}
    u[k]\\ \mathcal{X}_j[k]
\end{bmatrix},\;\text{where}\;\Lambda_j \triangleq \hat{X}_{j,n+1,T}
\begin{bmatrix}
U_{n,T}\\
\hat{X}_{j,n,T}
\end{bmatrix}\ssymbol{2}. \quad \square
\end{equation}
\end{lemma}

The proof of Lemma \ref{lem:data_OL} is in Appendix \ref{app3}. Lemma \ref{lem:data_OL} states that when the rank condition \eqref{eq:PE} is satisfied by the data $\mathcal{I}_T$, then \eqref{eq:SS_con_form} has an equivalent data-driven representation \eqref{data:OL}. An equivalent and simpler method to check if \eqref{eq:PE} holds was given in \citet[Lemma 1, and (81)]{de2019formulas} which requires checking if the input $u$ is persistently exciting of a certain order. This equivalent result is next recalled by including a remark that the observability of the data-generating matrices is a necessary condition for \eqref{eq:PE} to hold: highlighting the necessity of Assumption \ref{assum:q_sen_obsv}.
\begin{lemma}\label{lem:rank_obsv}
Let the input $u_{[n,n+T-1]}$ with $T\geq (m+1)\tilde{n}$ be persistently exciting of order $\tilde{n}$ as defined in Lemma \ref{lem:data_OL}, where $\tilde{n}=(m+N-M)n+1$. Then for a given $j \in \left\{1,\dots,{N \choose N-M}\right\}$, \eqref{eq:PE} cannot hold in the absence of attacks, if the tuple $(A,C_{{\mathcal{J}}_{j}})$ is not observable and $n < N-M+1$. $\hfill \square$
\end{lemma}
The proof of Lemma \ref{lem:rank_obsv} is given in Appendix \ref{app2}. Using this data-driven representation derived in Lemma \ref{lem:data_OL}, the algorithm to identify the attack-free sensors is described next.
\subsection{Attack identification of slowly switching attacks}\label{sec22}
{\color{red} Sri: I did not change anything in this subsection}
This section aims to identify the attack-free sensors online, using the open-loop representation in \eqref{data:OL}. To this end, consider the open-loop (offline) data consisting of inputs $u$ and measurements $\left\{z_1,z_2,\dots,z_{{N \choose N-M}}\right\}$. Using the data, construct the data matrices in \eqref{data_matrices}, \eqref{data_matrices1}, \eqref{data_matrices2}, and $\Lambda_j$ for $j \in \{1,2,\dots, {N\choose N-M} \}$. Now, the matrix $\Lambda_j$ is the model for the operator, and all input $u$ and attack-free output $y$ trajectories that satisfy \eqref{P} also satisfy \eqref{data:OL} 

Now, consider the online measurements 
\begin{equation} \label{eq:online_meas}
    \tilde{z}_{j}=\tilde{y}_{\mathcal{J}_{j}}, \quad j\in\left\{1,2,\dots, {N\choose N-M} \right\}, 
\end{equation}
where $\tilde{y}_{\mathcal{J}_{j}}$ denotes the stacking of $\tilde{y}_{i}$ for $i\in\mathcal{J}_{j}$. Note that the online measurements $\tilde{z}_{j}$ can also be written as $\tilde{z}_{j}=z_j + a_{{\mathcal{J}_{j}}}$ and are potentially corrupted. By construction, there is one signal $\tilde{z}_j$ for $ j\in \{1,2,\dots, {N\choose N-M} \}$ that is attack-free. Then, for a given input $u$, the data-driven open-loop (offline) model given in \eqref{data:OL} explains the attack-free sensor measurements $\tilde{z}_{j}$. Motivated by the above argument, we apply new test input signals (say $\underline{u}$) of length $T_1$, collect the corresponding outputs $\underline{y}$ and construct the new data set 
\begin{equation}\label{eq:test_data}
\underline{\mathcal{I}}_{T_1} \triangleq \left\{\underline{u}_{[0, T_1-1]},\underline{y}_{[0, T_1-1]} \right\}.
\end{equation}
As before, let us construct the data matrices in \eqref{data_matrices} using the test data $\underline{\mathcal{I}}_{T_1}$ in \eqref{eq:test_data}. Let us represent the data matrices as $\underline{U}_{k+n,T_1}, \underline{\hat{X}}_{j,k+n,T_1},$ and $\underline{\hat{X}}_{j,k+n+1,T_1}$. Then, the attack-free sensors (indexed by $j^* \in \left\{1,2,\dots, {N\choose N-M} \right\}$) at any time instant $k\in\mathbb{Z}$ are given by 
\begin{equation}\label{eq:attack_cond}
    j^*[k] \in \underset{{j\in \left\{1,2,\dots, {N \choose N-M} \right\}}}{\arg\min} \Bigg|\Bigg| \underline{\hat{X}}_{j,k+n+1,T_1}-\Lambda_j\begin{bmatrix}
        \underline{U}_{k+n,T_1}\\
        \underline{\hat{X}}_{j,k+n,T_1}
    \end{bmatrix}\Bigg|\Bigg|_2.
\end{equation}
The procedure described above is depicted as an algorithm in Algorithm \ref{alg1}. Once the attack-free sensors have been identified, the sensors under attack are allowed to switch. That is, the attacks cannot switch while the \textit{test} data of length $T_1$ is being collected. Combining the above arguments, the following result is stated.
\begin{prop}\label{prop1}
Consider the plant \eqref{P} under Assumption \ref{assum:M-attacks} and \ref{assum:q_sen_obsv}. Then ${j^*}$ obtained from Algorithm \ref{alg1} is the vector of attack-free sensors when the attack switches at a frequency less than $1/T_1$. $\hfill \square$
\end{prop}
% {\color{red} Michelle: the proof is not complete. Can you please make sure that the the slowly switching attack is incorporated in your proof. As it is now, this is not stated clearly.}
The proof of Proposition \ref{prop1} is given in Appendix \ref{app5}. The result stated in Proposition \ref{prop1} relies on the fact that the plant \eqref{P} has an equivalent data-driven representation in \eqref{data:OL}. As stated in Lemma \ref{lem:data_OL}, the observability of the data generating system is a necessary condition for the rank condition \eqref{eq:PE} to hold, which is in turn necessary for the existence of the data-driven representation \eqref{data:OL} as stated in Lemma \ref{lem:data_OL}. Thus, Assumption \ref{assum:q_sen_obsv} is a necessary condition for the data-driven representation \eqref{data:OL} to be equivalent to \eqref{P}, and for Algorithm \eqref{alg1} to work. The next section provides a discussion on the identification of attack-free sensors without access to $\mathcal{I}_T$ in the presence of sensor delay attacks.
\begin{algorithm}
\caption{Algorithm to identify attack-free sensors under slowly switching sensor attacks}
\textbf{Begin algorithm}
\begin{enumerate}
\item (Offline) Using $\mathcal{I}_T$, construct $\Lambda_j, \; \forall j \in j\in \left\{1,2,\dots, {N \choose N-M} \right\}$ from Lemma \ref{lem:data_OL}.
\item (Online) Apply \textit{test} input data of length $T_1$, collect the corresponding output data, and construct the matrices $\underline{U}_{k+n,T_1}, \underline{\hat{X}}_{j,k+n,T_1},$ and $\underline{\hat{X}}_{j,k+n+1,T_1}$ for all $j \in j\in \left\{1,2,\dots, {N \choose N-M} \right\}$. 
\item (Online) Determine $j^*[k]$ from \eqref{eq:attack_cond}.
\end{enumerate}
\KwResult{Attack free sensors: $j^*$}
\textbf{End algorithm}
\label{alg1}
\end{algorithm}



==> Archive/Identification-27Nov23.tex <==
The overall scheme proposed for attack identification is as follows. Using the attack-free data set ($\mathcal{I}_{T}$), and by building on the works of \cite{de2019formulas}, an equivalent data-based representation is constructed for the plant \eqref{P}. This equivalent representation is then used to identify the attack-free sensors when the plant is controlled online. 
\subsection{Learning the data-driven open-loop model}
To derive an equivalent open-loop representation for the plant \eqref{P}, recall from Definition \ref{def:q_sen_obsv} that $\mathcal{J}_Q$ represents a subset of $ \{1,2,\dots,N\}$ with cardinality $Q$, given that $Q\leq N$. Then, let $\bar{\mathcal{J}}_Q$ be the set of all possible $\mathcal{J}_Q$ for a given $Q$. For any given (set) element  of $\bar{\mathcal{J}}_Q$ (denoted by $\bar{\mathcal{J}}_{Q,j}$), let $C_{\bar{\mathcal{J}}_{Q,j}}$ be a matrix obtained by stacking all the matrices $C_i,i\in \bar{\mathcal{J}}_{Q,j}$, and let the stacked projection of $\bar{\mathcal{J}}_{Q,j}$ on $\tilde{y} $ be denoted by $z_j$. Let plant in \eqref{P} with output $z_j[k]$ be described as follows
\begin{equation}\label{eq:SS_con_form}
x[k+1]=Ax[k]+Bu[k], \quad z_j[k]=C_{\bar{\mathcal{J}}_{Q,j}}x[k],\;j \in \Omega, \Omega \triangleq \{1,\dots,{N \choose Q}\}
\end{equation}
where $z_j[k]\in\mathbb{R}^{Q}$. Note that \eqref{P} and \eqref{eq:SS_con_form} are equivalent since their input output trajectories match. In \eqref{eq:SS_con_form}, the operator knows the values of $N$ and $M$. To construct a data-based representation of the plant \eqref{eq:SS_con_form} (or equivalently \eqref{P}) using $\mathcal{I}_{T}$, define 
\begin{equation}\label{data_matrices0}
\hat{X}_{j,n,T} \triangleq  \begin{bmatrix}
        Z_{j,0,n,T}\\
        \hline 
        U_{0,n,T}\\
    \end{bmatrix},\; \mathcal{X}_{j}[k]^T \triangleq
\setlength{\dashlinegap}{0.5pt}
\begin{bmatrix}[ccc:ccc] z_{j}^T[k-n]&...&z_j^T[k-1]& u^T[k-n]&...& u^T[k-1]\end{bmatrix}.
\end{equation}
Then the operator constructs the following matrices from the data. 
\begin{align}
    U_{n,T}&=\begin{bmatrix}
        u[n] & u[n+1]& \dots & u[n+T-1]
    \end{bmatrix} \label{data_matrices}\\
    \hat{X}_{j,n,T}&=\begin{bmatrix}
        \mathcal{X}_{j}[n] & \mathcal{X}_{j}[n+1]& \dots & \mathcal{X}_{j}[n+T-1]
    \end{bmatrix} \label{data_matrices1}\\
    \hat{X}_{j,n+1,T}&=\begin{bmatrix}
        \mathcal{X}_{j}[n+1] & \mathcal{X}_{j}[n+2]& \dots & \mathcal{X}_{j}[n+T]
    \end{bmatrix} \label{data_matrices2}
\end{align}
Note that the state $\mathcal{X}_j$ in contains the history of past inputs and past outputs of length $n$. Thus there is an offset of length $n$ whilst constructing the data matrices \eqref{data_matrices}. Now the following result is stated from \citet[Theorem 1, Lemma 2]{de2019formulas}.
\begin{lemma}\label{lem:data_OL}
For any given $j \in \Omega$, let
\begin{equation}\label{eq:PE}
    \text{rank}\begin{bmatrix}
        U_{n,T}\\\hat{X}_{j,n,T}
    \end{bmatrix}=m(n+1)+Qn,
\end{equation}
with $T\geq (m+1)\tilde{n}$ where $\tilde{n}\triangleq (m+Q)n+1$. Then \eqref{eq:SS_con_form} has the equivalent data-driven representation in \eqref{data:OL}, where $\ssymbol{2}$ denotes the right inverse.
\begin{equation}\label{data:OL}
\mathcal{X}_j[k+1]=\Lambda_j\begin{bmatrix}
    u[k]\\ \mathcal{X}_j[k]
\end{bmatrix},\;\text{where}\;\Lambda_j \triangleq \hat{X}_{j,n+1,T}
\begin{bmatrix}
U_{n,T}\\
\hat{X}_{j,n,T}
\end{bmatrix}\ssymbol{2}. \quad \square
\end{equation}
\end{lemma}

The proof of Lemma \ref{lem:data_OL} is in Appendix \ref{app3}. Lemma \ref{lem:data_OL} states that when the rank condition \eqref{eq:PE} is satisfied by the data $\mathcal{I}_T$, then \eqref{eq:SS_con_form} has an equivalent data-driven representation \eqref{data:OL}. An equivalent and simpler method to check if \eqref{eq:PE} holds was given in \citet[Lemma 1, and (81)]{de2019formulas} which requires checking if the input $u$ is persistently exciting of a certain order. This equivalent result is next recalled by including a remark that the observability of the data-generating matrices is a necessary condition for \eqref{eq:PE} to hold: highlighting the necessity of Assumption \ref{ass1}.
\begin{lemma}\label{lem:rank_obsv}
Let the input $u_{[n,n+T-1]}$ be persistently exciting of order $\tilde{n}$ as in Lemma \ref{lem:data_OL}, where $\tilde{n}=(m+Q)n+1$. Then for a given $j \in \Omega$, \eqref{eq:PE} cannot hold in the absence of attacks, if the tuple $(A,C_{\bar{\mathcal{J}}_{Q,j}})$ is not observable and $n < Q+1$. $\hfill \square$
\end{lemma}
The proof of Lemma \ref{lem:rank_obsv} is given in Appendix \ref{app2}. Using this data-driven representation derived in Lemma \ref{lem:data_OL}, the algorithm to identify the attack-free sensors is described next.
\subsection{Attack identification of slowly switching attacks}\label{sec22}
This section aims to identify the attack-free sensors online, using the open-loop representation in \eqref{data:OL}. To this end, consider the set of inputs and measurements $\{z_1,z_2,\dots,z_{{N \choose Q}}\}$. Using the measurements, construct the data matrices in \eqref{data_matrices}, \eqref{data_matrices1}, \eqref{data_matrices2}, and $\Lambda_j, \forall j \in \Omega$. Now, the matrix $\Lambda_j$ is the model for the operator, and all input-output trajectories that satisfy \eqref{P} also satisfy \eqref{data:OL} 

By construction, there exists one signal $z_j, j\in \Omega$ that is attack-free. Then, if we apply inputs to the plant (online) and the model $\Lambda_j$, the outputs are the same for the attack-free sensor pairs and different for the attacked sensor pairs. Motivated by the above argument, apply new test input signals (say $\underline{u}$) of length $T_1$, collect the corresponding outputs $\underline{y}$ and construct the new data set 
\begin{equation}\label{eq:test_data}
\underline{\mathcal{I}}_{T_1} \triangleq \{\underline{u}_{[0, T_1-1]},\underline{u}_{[0, T_1-1]} \}.
\end{equation}
As before, let us construct the data matrices in \eqref{data_matrices} using the test data $\underline{\mathcal{I}}_{T_1}$ in \eqref{eq:test_data}. Let us represent the data matrices as $\underline{U}_{k+n,T_1}, \underline{\hat{X}}_{j,k+n,T_1},$ and $\underline{\hat{X}}_{j,k+n+1,T_1}$. Then, the attack-free sensors (denoted by $j^* \in \Omega$) at any time instant are given by 
\begin{equation}\label{eq:attack_cond}
    j^*[k] \in \arg\min_{j\in \Omega} \Bigg|\Bigg| \underline{\hat{X}}_{j,k+n+1,T_1}-\Lambda_j\begin{bmatrix}
        \underline{U}_{k+n,T_1}\\
        \underline{\hat{X}}_{j,k+n,T_1}
    \end{bmatrix}\Bigg|\Bigg|_2
\end{equation}
The procedure described above is depicted as an algorithm in Algorithm \ref{alg1}. Once the attack-free sensors have been identified, the sensors under attack are allowed to switch. That is, the attacks cannot switch while the \textit{test} data of length $T_1$ is being collected. Combining the above arguments, the following result is stated.
\begin{prop}\label{prop1}
Consider the plant \eqref{P} under Assumption \ref{ass_ctrb} and \ref{ass1}. Then ${j^*}$ obtained from Algorithm \ref{alg1} is the vector of attack-free sensors when the attack switches at a frequency less than $1/T_1$. $\hfill \square$
\end{prop}
The proof of Proposition \ref{prop1} is given in Appendix \ref{app5}. The result stated in Proposition \ref{prop1} relies on the fact that the plant \eqref{P} has an equivalent data-driven representation in \eqref{data:OL}. As stated in Lemma \ref{lem:data_OL}, the observability of the data generating system is a necessary condition for the rank condition \eqref{eq:PE} to hold, which is in turn necessary for the existence of the data-driven representation \eqref{data:OL} as stated in Lemma \ref{lem:data_OL}. Thus, Assumption \ref{ass1} is a necessary condition for the data-driven representation \eqref{data:OL} to be equivalent to \eqref{P}, and for Algorithm \eqref{alg1} to work. The next section provides a discussion on the identification of attack-free sensors without access to $\mathcal{I}_T$ in the presence of sensor delay attacks.
\begin{algorithm}
\caption{Algorithm to identify attack-free sensors under slowly switching sensor attacks}
\textbf{Begin algorithm}
\begin{enumerate}
\item (Offline) Using $\mathcal{I}_T$, construct $\Lambda_j, \; \forall j \in \Omega$ from Lemma \ref{lem:data_OL}.
\item (Online) Apply \textit{test} input data of length $T_1$, collect the corresponding output data, and construct the matrices $\underline{U}_{k+n,T_1}, \underline{\hat{X}}_{j,k+n,T_1},$ and $\underline{\hat{X}}_{j,k+n+1,T_1}$ for all $j \in \Omega$. 
\item (Online) Determine $j^*[k]$ from \eqref{eq:attack_cond}.
\end{enumerate}
\KwResult{Attack free sensors: $j^*$}
\textbf{End algorithm}
\label{alg1}
\end{algorithm}

==> Archive/Online-5Dec23.tex <==
In the previous section, we discussed the identification of attacks when we have access to offline data of fixed length. However, in some scenarios, offline data might not be available. Thus in this section, we discuss cases in which attack identification can be performed without $\mathcal{I}_T$ before which we establish the following assumption. 
\begin{assumption}\label{ass_eq}
The plant \eqref{P} is at equilibrium $x[0]=0$ before the attack commences. $\hfill \triangleleft$
\end{assumption}
Assumption \ref{ass_eq} does not introduce any loss of generality due to the following reasons. In reality, the plant is usually stabilized locally with a feedback controller (for safety), and a network controller is used to improve performance, change set points, etc. This approach of having two controllers is adopted in the literature \citep{lin2022plug,lin2023secondary} to avoid stability issues due to packet dropouts, delays, bandwidth limitations, etc \citep{hu2007stability}. Thus, the stable plant (along with the local controller) reaches an equilibrium from any non-zero initial condition satisfying Assumption \ref{ass_eq}. Such assumptions are also common in the literature \citep{wang2020neural,nonhoff2022online}.
\subsection{Network delay attacks}
As mentioned in the introduction, there are different kinds of attacks studied in the literature which include stealthy data-injection attacks, replay attacks, zero-dynamics attacks, covert attacks, and many more \citep{teixeira2015secure}. One of the attacks which have not been studied intensively is time delay attacks \citep{bianchin2018time,wigren2023line}. Delay attacks are shown to destabilize power grids \citep{korkmaz2016ics}, however, their detection schemes are not well developed. In this paper, we first represent delay attacks as follows 
\begin{equation}
    \tilde{y}_i[k] = y_i[k-\tau_i], \tau_i \geq 0, \tau_i \in \mathbb{Z}, \forall i \in \{1,\dots,N\}
\end{equation}
where $\tilde{y}_i[k]$ is the delayed measurement received by the operator. Next, we attempt to identify the sensors which are free of delay attacks. However, we consider single-input systems for simplicity. We start the discussion by defining relative degree.
\begin{definition}\label{def:rd}
Relative degree $(r_j)$ of the system $\Sigma_j=(A,B,C_j,0), j\in\{1,\dots,N\}$ is defined as\vspace{-5pt} 
\begin{equation}
r_j \triangleq 1+\min \{ i \;| C_jA^iB \neq 0, i \geq 0 \}. \quad \triangleleft
\end{equation}
\end{definition}
The relative degree of $\Sigma_j$ denotes the amount of time delay before the input $u[k]$ appears in its output $y_j[k]$. For instance, consider a system with a feed-through term $D \neq 0$, then the input $u[k]$ immediately appears in the output making the relative degree of $\Sigma$ zero. Next, we establish the following assumptions. 
\begin{assumption}\label{ass2}
We do not have offline data $\mathcal{I}_T$, and we know the value of $r_j$, $\forall \; j\in\{1,\dots,N\} \hfill \triangleleft$
\end{assumption}
In other words, we assume that we have some degree of knowledge about the plant in terms of the relative degree (instead of attack-free data). For instance, the relative degree can be obtained from the physics of the plant. That is, if the operator knows the physics of the plant but does not know the exact parameters of the plant (as considered in \cite{de2023learning}), then the operator can infer relative degrees. With this knowledge of the relative degrees, when Assumption \ref{ass_ctrb}, \ref{ass1}, \ref{ass_eq} and \ref{ass2} are satisfied, we next describe an algorithm for identification of delay attack-free sensors.

Let us apply a non-zero input signal of unit length (approximate impulse) and collect the corresponding outputs. Since the input is non-zero, and the plant is at equilibrium before the attack, the outputs corresponding to the sensor $y_j$ should be non-zero after $r_j$ amount of time. If the output of the sensor $y_j$ is zero after $r_j$ amount of time, then the corresponding sensor is under attack. Then, the attack-free sensors (denoted by $j^* \in \Omega$) at any time instant are given by 
\begin{align}\label{eq:att_delay}
    j^*[k] &\in \arg\min_{j\in \Omega} \left\{ \sigma_j - r_j\right\}, \quad \sigma_j \in \min \{k \vert Y_{j,0,T}[1,k] \neq 0\}.
\end{align}
The idea behind \eqref{eq:att_delay} is explained as follows: The second equation determines the first column of $Y_j$ which is non-zero. Ideally, when there is no attack, the first non-zero column of $Y_j$ would be $r_j$. The procedure described above is depicted as an algorithm in Algorithm \ref{alg1}. 

In this section, akin to the experimental design techniques for data-driven learning \citep{de2021designing}, we proposed input design techniques for attack detection. In the next section, we briefly discuss the online identification of replay attacks. 
\begin{algorithm}
\caption{Algorithm to identify delay attack-free sensors}
\textbf{Begin algorithm}
\begin{enumerate}
\item Apply \textit{non-zero} input vector of (unit) length $1$.
\item Collect the corresponding outputs and construct the matrices $Y_{j,0,T}, \forall j \in \{1,\dots, {N}\}$ where $T \geq  \max_j{r_j}$.
\item Determine $j^*$ from \eqref{eq:att_delay}
\end{enumerate}
% \item \textbf{Result:}
\KwResult{Attack free sensors: $j^*$}
\textbf{End algorithm}
\vspace{-15pt}
\label{alg2}
\end{algorithm}
\subsection{Replay attacks}
In this section, we consider the case of replay attacks \cite{teixeira2015secure}. We consider an adversary who has recorded the sensor measurements which are constants. These constants can correspond to the equilibrium point (Assumption \ref{ass_eq}) or any other operating point. For instance, if the local controller is designed for reference tracking, the outputs might correspond to the constant reference trajectory. We represent replay attacks as 
\begin{equation}\label{replay}
    \tilde{y}_i[k] = c_i, \forall i \in \{1,\dots,N\}
\end{equation}
where $c_i$ is a constant unknown to the operator. Another approach to motivate attacks in \eqref{replay} is as follows. Under Assumption \ref{ass1}, let us consider the plant is under constant bias injection attacks \citep{teixeira2015secure,farraj2017impact,jin2022distributed}. Then, the attack can be modeled as \eqref{replay} where the $c_i$ denotes the bias injected into sensor $i$. The effect of bias injection attacks (also when the bias is slowly increasing) on experimental setups was also recently studied \citep{kedar2023evaluation}. Next, we are interested in detecting the sensors that are replay attack-free.  

Motivated by the discussion around Algorithm \ref{alg1}, let us apply test input signals (say $\underline{u}$) of length $T_1$, collect the corresponding outputs $\underline{y}$ and construct the data set $\underline{\mathcal{I}}_{T_1}$ in \eqref{eq:test_data}. As before, let us construct the data matrices in \eqref{data_matrices} using the test data $\underline{\mathcal{I}}_{T_1}$ in \eqref{eq:test_data}. Let us represent the data matrices as $\underline{U}_{k+n,T_1}, \underline{\hat{X}}_{j,k+n,T_1},$ and $\underline{\hat{X}}_{j,k+n+1,T_1}$. Then, we present the following result

\begin{lemma}\label{lem:replay}
Consider the plant \eqref{P} under replay attacks \eqref{replay}, Assumption \ref{ass1}, and Assumption \ref{ass_eq}. Then, if the sensor pair $j$ is under replay attack, the following rank condition 
\begin{equation}\label{rank:replay}
    \text{rank}\begin{bmatrix}
        \underline{U}_{k+n,T_1},\\ \underline{\hat{X}}_{j,k+n,T_1},
    \end{bmatrix}=m(n+1)+Qn,
\end{equation}
with $T_1\geq (m+1)\tilde{n}, k\in \mathbb{Z}$ and $\tilde{n}\triangleq (m+Q)n+1$ cannot hold. $\hfill \square$
\end{lemma}
The proof of Lemma \ref{lem:replay} is in Appendix \ref{App6}. Lemma \ref{lem:replay} says that, if the sensors are under replay attack, and we design the inputs such that rank condition in \eqref{rank:replay} can be used as a test to detect replay attacks. Thus in this section, we proposed algorithms to detect attacks online without using the offline attack-free data $\mathcal{I}_T$. We also note that, by applying the test inputs to detect attacks, we perturb the system from its equilibrium and lose performance similar to other detection techniques in the literature \citep{mo2015physical}.

==> Archive/Problem-27Nov23.tex <==
Consider an LTI State-space (SS) model of the plant ($\mathcal{P}$) described as:
\begin{equation}\label{P}
\mathcal{P}: 
    \begin{aligned}
x[k+1]&=Ax[k]+Bu[k], \quad 
y_i[k]= C_ix[k],\;i \in \{1,\dots,N\},
\end{aligned}
\end{equation}
where the state of the plant is represented by $x[k] \in \mathbb{R}^n$, the control input applied to the plant is represented by $u[k] \in \mathbb{R}^m$, the output of the noise-free sensor $i, i \in \{1,\dots,N\}$ is represented by $y_i[k] \in \mathbb{R}$ and the matrices are of appropriate dimension. Without loss of generality, it is assumed that each sensor is of unit dimension, and the following notation is alternatively used for simplicity
\begin{equation}
y[k] =Cx[k], \quad y[k]= \begin{bmatrix}
        y_1[k]^T & y_2[k]^T & \dots & y_N[k]^T
    \end{bmatrix}^T, \quad
    C=\begin{bmatrix}
        C_1^T & C_2^T & \dots & C_N^T
    \end{bmatrix}^T.
\end{equation}
As shown in Figure.~\ref{fig:NCS}, the sensor values are transmitted over the network for control/monitoring purposes. Such a setup, where only the sensor values are transmitted over the network, is considered for simplicity as in some other works in the literature \citep{feng2017resilient,teixeira2018detection}. Since the sensor values are transmitted over a network, they are prone to cyber-attacks. Thus, this paper considers an adversary injecting malicious signals into the sensor communication channel. Next, some assumptions are established.
\begin{assumption}\label{ass_ctrb}
    The tuple $(A,B)$ is controllable. $\hfill \triangleleft$
\end{assumption}
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{NCS.pdf}
    \caption{Networked control system under sensor attacks.}
    \label{fig:NCS}
    \vspace{-15pt}
\end{figure}
To establish some assumptions on the observability of the plant, similar to \cite{chong2015observability}, the definition of $Q$-sensor observability is introduced next.
\begin{definition}[$Q$-sensor observability]\label{def:q_sen_obsv}
Let $\mathcal{J}_Q$ represent any subset of $\{1,2,\dots,N\}$ with cardinality $Q$, given that $Q<N$. Then, plant \eqref{P} is $Q-$sensor observable if for every set $\mathcal{J}_{Q}$, the tuple $(A,C_{\mathcal{J}_Q})$ is observable where $C_{\mathcal{J}_Q}$ is a matrix obtained by stacking the matrices $C_i,i\in \mathcal{J}_Q$. $\hfill \triangleleft$
\end{definition}
Definition \ref{def:q_sen_obsv} states that an LTI system is $Q$-sensor observable if the system is observable for every combination of $Q$ sensors. Next, we establish the following assumption.
\begin{assumption}\label{ass1}
The plant \eqref{P} is $Q$-sensor observable, where $Q\triangleq N-M, Q > 0$, and $M$ represents the number of sensors under attack. In the rest of the sequel, let $Q\triangleq N-M. \hfill \triangleleft$
\end{assumption}
Here, the value of $M$ represents an upper bound on the number of sensors that the operator believes are susceptible to attack. For instance, it can represent the sensor channels for which the encryption key has not been updated recently. The necessity of the Assumption \ref{ass1} is explained as follows. Firstly, Assumption \ref{ass1} is necessary to derive a data-driven representation of the plant, as explained later, Secondly, the identified attack-free sensors are generally used to design a controller that requires observable sensors. Additionally, such assumptions were also made in secure state estimation literature \citep{chong2015observability}. Next, the attack scenario is explained in detail. 
\subsection{Data injection attack scenario}
As depicted in Figure.~\ref{fig:NCS}, an adversary injects malicious data into the sensors and is represented by
\begin{equation}\label{att_vec}
\Tilde{y}[k]=y[k]+a[k], \quad a[k]=\begin{bmatrix}
    a_1^T[k] & a_2^T[k] &  \dots & a_N^T[k] 
\end{bmatrix}^T
\end{equation}
where $\Tilde y$ represents the attacked sensor signal received by the operator, and $a_i$ represents the attack signal on sensor channel $i$, which is assumed to be Lebesgue measurable. In particular, three attack strategies are considered in this paper and are explained next. 
\begin{enumerate}
\item \textit{Slowly switching sensor attacks} are of arbitrary magnitudes, and switch (the attacked sensors) at a low frequency but only corrupt at most $M$ sensors at any given time.
\item \textit{Sensor-network delay attacks} introduces arbitrary but bounded delays in at most $M$ sensors.
\item \textit{Sensor replay attacks} records sensor values and replays them in at most $M$ sensors.
\end{enumerate}
Note that slowly switching sensor attacks are more general than the other two attacks. Next, the main objective of this paper is stated.
\subsection{Problem formulation}
As shown in Figure.~\ref{fig:NCS}, consider an operator located on the other side of the network that does not know the system matrices $A, B$, and $C$. Such a setup is considered to analyze the worst-case scenario. However, the operator has access to the offline attack-free input-output trajectories 
\begin{equation}\label{IT}
    \mathcal{I}_{T}=\{u_{[0,T-1]},{y}_{[0,T-1}\}
\end{equation}
of length $T$ (where $T$ is sufficiently large). The data $\mathcal{I}_T$ is assumed to be collected (in open-loop) before the plant is controlled online and thus is attack-free. Such assumptions are also common in the literature (see \citet[Assumption 2.2]{liu2023online} and references therein).

When the plant data is transmitted online (the sensor data is transmitted over the network) for control and monitoring purposes, the sensor data is possibly corrupted. Then the aim of the operator (and this paper) is as follows: when the plant is controlled/monitored online, identify the attack-free sensors using \textit{only} the knowledge of $\mathcal{I}_{T}$ in \eqref{IT}. To this end, we describe an algorithm that solves the sensor identification problem for slowly switching sensor attacks in Section \ref{sec:identify}. In Section \ref{sec:online}, we describe an algorithm that solves the sensor identification problem for delay and replay attacks.

==> Switch.tex <==
In the previous sections, we considered that the attacked sensors are constant ($M$) and do not change over time. In this section we consider that the attacked sensor channels slowly change over time, however, we still assume that the number of attacked sensor channels is at most $M$.

\begin{algorithm}
\caption{Algorithm to stabilize \eqref{P} using data under slowly switching sensor attacks}
\textbf{Begin algorithm}
\begin{enumerate}
\item[]\underline{Attack identification:}
\item Apply input of length $T$ which satisfy \eqref{eq:PE} and construct $\Lambda_j, \; \forall j \in \{1,2,\dots,{N \choose Q}\}$.
\item Collect new data points of arbitrary length $T_1$ and construct the matrices $\underline{U}_{n,T_1}, \underline{\hat{X}}_{j,n,T_1},$ and $\underline{\hat{X}}_{j,n+1,T_1}$ for all $j$. 
\item Determine $j^*$ from \eqref{eq:attack_cond}.
\item[]\underline{Attack resilient control design:}
\item Determine the controller $K_{j^*}$ from \eqref{eq:design_LMI} and \eqref{eq:design_K}.
\item Save the tuple $j^*,\Lambda_{j^*}$ and $K_{j^*}$ to the list $\mathcal{L}$.
\item Apply the controller $K_{j^*}$ in feedback.
\end{enumerate}
\underline{Attack Monitoring:}\\
\While{true}{
At each time step, construct $\mathcal{X}_{j^*}[k]$ and determine $$\sigma_a = \Bigg|\Bigg| \mathcal{X}_{j^*}[k]-\Lambda_{j^*}\begin{bmatrix} u[k-1]\\\mathcal{X}_{j^*}[k-1] \end{bmatrix}\Bigg|\Bigg|_2$$
\If{$\sigma_a \geq \epsilon$}{
\textbf{(a)} Remove the feedback controller.\\
% \textbf{(a)} Collect new data points of arbitrary length $T_1$ and construct the matrices $\underline{U}_{n,T_1}, \underline{\hat{X}}_{j,n,T_1},$ and $\underline{\hat{X}}_{j,n+1,T_1}$ for all $j$. \\
\textbf{(b)} Construct $\mathcal{X}_j[k]$ and $\mathcal{X}_j[k-1], \forall j\in \mathcal{L}_J$ and determine 
$$\sigma_b =\min_{j\in \mathcal{L}_{J}} \Bigg|\Bigg| \mathcal{X}_{j}[k]-\Lambda_{j}\begin{bmatrix} u[k-1]\\\mathcal{X}_{j}[k-1] \end{bmatrix}\Bigg|\Bigg|_2$$
where $\mathcal{L}_J$ represents the elements of $j^*$ belonging to the list $\mathcal{L}$ \\
\textbf{(c)} If $\sigma_b < \epsilon $ for some argument $j^{**}$, set $j^*=j^{**}$ and go to step $6$.\\
\textbf{(d)} If $\sigma_b \geq \epsilon$, go to step $1$.
}
}
\textbf{End algorithm}
\label{alg2}
\end{algorithm}

The algorithm for attack identification under slowly switching attacks is presented in Algorithm \ref{alg2}. The idea behind the algorithm is as follows: let us consider that $M$ sensors are under attack. In order to identify the attack free-sensors, and stabilize the system, Algorithm \ref{alg2} performs the same procedure as for static attack channels in Steps $1$ through $6$. When we identify an attack-free sensor pair $j^*$, we save the corresponding matrix $\Lambda_{j^*},$ and $K_{j^*}$ to a list $\mathcal{L}$. And we assume that the attacked sensor channels do not switch during this phase of attack identification and control design. 

Once the designed stabilizing controller is applied in feedback, the attacked sensor channels are allowed to switch. However, when the attacked channels do not switch, the states of the system \eqref{eq:CL} obeys \eqref{data:OL} when $j=j^*$. Thus, the value of $\sigma_a$ is close to $0$ if the attacks do not switch, and a larger $\sigma_a$ denotes that the attack has switched channels. 

Once the attacked sensor channels switch, we check if the outputs corresponding to the sensor pairs $j\in \mathcal{L}_J$ are attack-free. In other words, we check if the attacker has switched back to a previously attacked sensor channel. If yes, then we apply the corresponding stabilizing controller previously designed. Else, we go back to attack identification. We explain this part next with an example. 

Consider a system with $N=3$ outputs, and $Q=1$-sensor observable. At first, if the sensors $\{2,3\}$ are under attack, we identify that sensor $1$ is attack-free, determine $\Lambda_1$ and save it to the list $\mathcal{L}$. Then the attack switches to sensors $\{1,3\}$. we identify that sensor $2$ is attack-free, determine $\Lambda_2$ and save it to the list $\mathcal{L}$. If the attack now switches back to $\{2,3\}$, we no longer have to reconstruct the matrix $\Lambda_1$ (steps 1 through 4 of Algorithm \ref{alg2}), since we already identified the attack-free $\Lambda_1$ in the first instance. We combine the above arguments into the following proposition. 

\begin{prop}\label{prop2}
Consider the open-loop system \eqref{data:OL} under Assumption \ref{ass1}. Then the following statements are true. 
\begin{enumerate}
    \item Algorithm \ref{alg2} stabilizes the open-loop system \eqref{data:OL} when the attack switches at a frequency less than $\frac{1}{T+T1+T_d}$, where $T_d$ is the time taken to execute steps $3$ through $6$ of Algorithm \ref{alg2}: construct the data matrices, identify the attack-free sensors, and solve the design LMI \eqref{eq:design_LMI}.
    \item With the attack switching at a frequency less than $\frac{1}{T+T1+T_d}$, let us consider that the attack has occurred at least once in every possible ${N \choose M}$ sensor channel. Then, Algorithm \ref{alg2} stabilizes the open-loop system \eqref{data:OL} when the attack switches at a frequency less than $\frac{1}{2T_e}$ where $T_e$ is the time required to execute one iteration of the while loop of the attack monitoring phase.$\hfill \square$
\end{enumerate}
\end{prop}

In Proposition \ref{prop2}, the first statement follows from the discussion before. That is, once we identify that the sensors under attack have switched, we need to inject PE input of length $T$, collect test data of length $T_1$, identify the clean sensors, and then construct and apply the stabilizing controller. And since the attacks do not switch during this data-collection and controller design phase, we can design the stabilizing controller. 

However, once the attack has occurred in all possible ${N \choose M}$ sensor channels, the controller will have access to the attack-free $\Lambda_j, j\in \{1,\dots,{N\choose Q}\}$ from the list $\mathcal{L}$. In other words, there always exists an attack-free state $\mathcal{X}_{(\cdot)}$, which \textit{should} evolve according to \eqref{data:OL} where the corresponding $\Lambda_{(\cdot)}$ are in the list $\mathcal{L}$. The logic behind the second statement is explained next with the same example before Proposition \ref{prop2}. 

Consider a system that has $N=3$ outputs, and the system is $Q=1$-sensor observable. At first, sensors $\{2,3\}$ are under attack. We identify the attack free $1$, determine $\Lambda_1$, $K_1$ and save it to the list $\mathcal{L}$. Then, when the attack switches to sensors $\{1,3\}$, we similarly construct $\Lambda_2, K_2$ and save them. Finally, when the attack switches to sensors $\{1,2\}$, we similarly construct $\Lambda_3, K_3$ and save them. Here, after the attack switches, in order to construct the stabilizing controller, we need to collect data of length $T+T1$. Thus we consider that the attack does not switch over the data-collection phase. 

Now, let us consider that the attack switches back to sensors $\{2,3\}$. Then, similar to before, we will be able to detect that sensor $1$ is the attack-free sensor. However, since we already know $K_1$, we do not have to inject PE inputs of length $T$. We directly implement the controller $K_1$. 

==> design.tex <==
In the previous section, we discussed a method to identify the sensors that are not under attack ($j^*$). Once these sensors have been identified, the problem is a standard output data-driven stabilization problem. 

To recall, the original problem was to design a controller that stabilizes the LTI plant \eqref{P}. Without any loss of generality, by virtue of the Lemma \ref{lem:SS_PMS}, we can reformulate the problem equivalently to designing a stabilizing controller for the ARX model \eqref{ARX} with $z_j=z_{j^*}$, or the corresponding extended state space model \eqref{eq:CL}. In other words, we are interested in designing a controller such that 
\begin{equation}\label{eq:stable}
\mathcal{X}_{j^*}[k+1]=\bar{A}_{j^*}\mathcal{X}_{j^*}[k] +\bar{B}_{j^*}u[k],
\end{equation}
where $\bar{A}_{j^*}$ and $\bar{B}_{j^*}$ are the matrices corresponding to the ARX model of $z_{j^*}$, is stable. To this end, inspired by \citep{de2019formulas}, we consider the controller of the following structure
\begin{align}\label{eq:controller}
y^c[k]+\Phi_{n}y^c[k-1&]+\dots\Phi_{1}y^c[k-n]=\\
&u^c[k]+\psi_{n}u^c[k-1]+\dots \psi_{1}u^c[k-n]
\end{align}
where $y^c[k]=u[k],$ and $u^c[k]=z_{j^*}[k]$. Then, the recall the following result from \citep[Corollary 2]{de2019formulas}.
\begin{lemma}\label{lem:design}
Let the following condition hold
\begin{equation}
    \text{rank}\begin{bmatrix}
        U_{0,T}\\ \hat{\mathcal{X}}_{j^*,n,T}
    \end{bmatrix}=m(n+1)+Qn.
\end{equation}
Then any matrix $\mathcal{Q}$ satisfying 
\begin{equation}\label{eq:design_LMI}
    \begin{bmatrix}
        \hat{\mathcal{X}}_{j^*,n,T}\mathcal{Q} &  \hat{\mathcal{X}}_{j^*,n+1,T}\mathcal{Q}\\
        \mathcal{Q}^T\hat{\mathcal{X}}_{j^*,n+1,T}^T & \hat{\mathcal{X}}_{j^*,n,T}\mathcal{Q}
    \end{bmatrix} \succ 0
\end{equation}
is such that the controller \eqref{eq:controller} with matrix coefficients
\begin{equation}\label{eq:design_K}
    \begin{bmatrix}
        \psi_{1} & \dots & \psi_{n} & -\Phi_1 & \dots & -\Phi_n
    \end{bmatrix}=U_0\mathcal{Q}(Z_{*,0}\mathcal{Q})^{-1} = K_{j^*}
\end{equation}
stabilizes the system \eqref{ARX}. $\hfill \square$
\end{lemma}

The above lemma describes an approach to design a controller that stabilizes \eqref{eq:stable}. Next, we provide a result that shows that the controller obtained also stabilizes \eqref{P}.

\begin{theorem}
        The output data-driven controller \eqref{eq:controller} stabilizes the SS model \eqref{P}.
\end{theorem}
\begin{proof}
    Consider the SS model \eqref{P}. Lemma \ref{lem:SS_PMS} states that there exists an ARX model equivalent to the SS model. Thus the input-output data obtained from the SS model \eqref{P} also satisfies the ARX \eqref{ARX} model and vice versa. Although the parameters of this equivalent ARX model (re-written in the extended state-space form \eqref{eq:stable}) are not known to the controller, Lemma \ref{lem:design} describes an approach to design a stabilizing controller for the ARX model and equivalently the SS model. This concludes the proof.
\end{proof}
